Training Certifiably Robust Neural Networks with Efficient Local Lipschitz Bounds

Certified robustness is a desirable property for deep neural networks in safety-critical applications, and popular training algorithms can certify robustness of a neural network by computing a global bound on its Lipschitz constant. However, such a bound is often loose: it tends to over-regularize the neural network and degrade its natural accuracy. A tighter Lipschitz bound may provide a better tradeoff between natural and certified accuracy, but is generally hard to compute exactly due to non-convexity of the network. In this work, we propose an efficient and trainable \emph{local} Lipschitz upper bound by considering the interactions between activation functions (e.g. ReLU) and weight matrices. Specifically, when computing the induced norm of a weight matrix, we eliminate the corresponding rows and columns where the activation function is guaranteed to be a constant in the neighborhood of each given data point, which provides a provably tighter bound than the global Lipschitz constant of the neural network. Our method can be used as a plug-in module to tighten the Lipschitz bound in many certifiable training algorithms. Furthermore, we propose to clip activation functions (e.g., ReLU and MaxMin) with a learnable upper threshold and a sparsity loss to assist the network to achieve an even tighter local Lipschitz bound. Experimentally, we show that our method consistently outperforms state-of-the-art methods in both clean and certified accuracy on MNIST, CIFAR-10 and TinyImageNet datasets with various network architectures.

==> sections/sec5_discussion.tex <==
\section{Discussion}
\begin{wrapfigure}{R}{0.4\textwidth}
    \centering
    \includegraphics[width=0.4\textwidth]{figures/poweriters.pdf}
    \caption{Histogram of number of iterations for power method to converge for the second last linear layer in 6C2F. }
    \label{fig:poweriter}
\end{wrapfigure}

\paragraph{Computational cost}
To compute the local lipschitz bound, we need to perform power iteration for every input and its feature maps at each layer. Let $u(t)$ be the singular vector computed by power iteration at iteration $t$, we stop power iteration when $|| u(t+1) - u(t) ||_2 \leq \expnumber{1}{-4}$. To analyze the computational cost, we plot the histogram of number of iterations for power method to converge for the second last layer in the 6C2F model in Figure \ref{fig:poweriter}. The average number of iterations for convergence is $1632$. The histograms for other layers are in Appendix.
To minimize the computational cost, we do not need to compute local lipschitz for inputs that can already be certified using global Lipschitz bound or can be attacked by adversaries. In practice, this typically rules out more than $50\%$ samples and can reduce computational cost by more than a half.


\yjcomment{add a figure comparing training and testing bcp loss for these two approaches.}



